Making Your First Choice: To Address Cold Start Problem in Vision Active Learning

Active learning promises to improve annotation efficiency by iteratively selecting the most important data to be annotated first. However, we uncover a striking contradiction to this promise: active learning fails to select data as efficiently as random selection at the first few choices. We identify this as the cold start problem in vision active learning, caused by a biased and outlier initial query. This paper seeks to address the cold start problem by exploiting the three advantages of contrastive learning: (1) no annotation is required; (2) label diversity is ensured by pseudo-labels to mitigate bias; (3) typical data is determined by contrastive features to reduce outliers. Experiments are conducted on CIFAR-10-LT and three medical imaging datasets (i.e. Colon Pathology, Abdominal CT, and Blood Cell Microscope). Our initial query not only significantly outperforms existing active querying strategies but also surpasses random selection by a large margin. We foresee our solution to the cold start problem as a simple yet strong baseline to choose the initial query for vision active learning. Code is available: https://github.com/c-liangyu/CSVAL

==> sections/7_others.tex <==
\newpage
{\jlblue 

\textbf{TODO}

1. Add better-better plots and results. Upload code for Zongwei. Use good colors for our method. Use dimmer or darker colors for baselines.
Put 20-60 xticks in main paper. 20-120 in appendix. No need to add correlation.
Save to csv file.

2. Contrastive learning initialization, not emergent. Add to Figure 6 only.

\textbf{3. Report both AUC and accuracy in future experiment. Done.}

\textbf{4. Unification of 2 criteria (intra- and inter-class framework). Change label uniformity to diversity.}

\textit{5. Additional natural image datasets, CIFAR-10 and CIFAR-100, only if we submit to CV/ML conferences.}

\textit{6. Motivation of hard-to-contrast data.}

\textit{7. Mathematics of cold-start problem, ask Guy.}

\textbf{8. Classifier training recipe of Figure 1, a classifier trained on test set. (See details in Appendix.) Done.}

\textbf{9. Figure 3 caption. See TMI paper Fig 18. Move PathMNIST and OrganAMNIST to appendix.}

\textbf{10. Related work titles (Sec 2.1) \noindent}

\textbf{11. Imprecise language and missing info?}

\textbf{12. Paste rebuttal and common reply answers. Done. Need discussion.}

\textbf{13. Clearer anotomy of causes of CSAL, in Intro sec.}

\textbf{14. Prepare questions for Guy. Done.}

\textbf{15. Check src dir. Done.}

\textbf{16. Design a MICCAI-style benchmark challenge, see Few-shot challenges.
https://cvpr21-nas.com/competition
https://aistudio.baidu.com/aistudio/competition/detail/64/0/introduction
}

The first impactful NAS dataset is NAS-BENCH-101. This is a huge table with 5M networks and their performances calculated by brute force. Its succeeder, NAS-BENCH-201 is also brute force.

[1902.09635] NAS-Bench-101: Towards Reproducible Neural Architecture Search
https://arxiv.org/abs/1902.09635

[2001.00326] NAS-Bench-201: Extending the Scope of Reproducible Neural Architecture Search
https://arxiv.org/abs/2001.00326

\textbf{See Coreset paper for greedy algorithm, maybe we can build a small form.}

Assume we use a small and hard dataset, (harder CIFAR-10). Performance not too high.

\textbf{OR, WE CAN put this as a semi-supervised learning problem with fixed labeling budget but free initial pool. See coreset challenges, if there is any. We describe a easy-to-understand problem statement in paper, as if we orgnaize a challenge about it.}

We have a public dataset.

Constraint:
1. Label budget is limited.

17. Calculate the purity of our query, Guy or tSNE method.

See whether we sample purple points in a green cluster.

The most common clustering purity metrics: purity and normalized mutual information.
https://nlp.stanford.edu/IR-book/html/htmledition/evaluation-of-clustering-1.html


\textbf{18. By Sept 22, Submit 8 page version to neurips-hill.github.io | NeurIPS 2022 Workshop on Human in the Loop Learning
https://neurips-hill.github.io/
}


\textit{IPMI 2021 AL paper} [2111.13069] Continual Active Learning Using Pseudo-Domains for Limited Labelling Resources and Changing Acquisition Characteristics
https://arxiv.org/abs/2111.13069

}

==> sections/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We discussed the limitations of this work in \S\ref{sec:conclusion}.} 
    % \answerYes{Extensive validation is largely done in classification tasks (justified in Lines 149--159 in \S\ref{sec:class_of_interest}).}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See \S\ref{sec:conclusion} for potential impacts. Negative impacts have not been identified.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
    \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{Our contributions are mostly empirical.}
    \item Did you include complete proofs of all theoretical results?
    \answerNA{Our contributions are mostly empirical.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
     \answerYes{Code is available at \href{https://anonymous.4open.science/r/cold\_start\_al-4D22/}{https://anonymous.4open.science/r/cold\_start\_al-4D22/} with detailed instructions. The data are described in \S\ref{sec:experiment} and Appendix~\ref{sec:implementation_appendix}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Details are presented in~\S\ref{sec:experiment} and Appendix~\ref{sec:training_recipe_contrastive_learning_appendix}--\ref{sec:training_recipe_medmnist_appendix}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Error bars and computation amount are reported. All results were based on at least 3 independent runs.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Our devices and the amount of computation are described in Appendix~\S\ref{sec:implementation_appendix}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We state the source of codes in Appendix~\ref{sec:implementation_appendix}.}
  \item Did you mention the license of the assets?
    \answerYes{The used code assets are under Apache License 2.0.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We would release our code as an asset. For peer-review, anonymous code is available at \href{https://anonymous.4open.science/r/cold\_start\_al-4D22/}{https://anonymous.4open.science/r/cold\_start\_al-4D22/}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Our empirical studies are solely based on five public datasets.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Our used five public datasets do not contain personally identifiable information or offensive content.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{Our experiments involve no human subjects and crowdsourcing.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{Our experiments involve no human subjects or crowdsourcing.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{Our experiments involve no human subjects or crowdsourcing.}
\end{enumerate}


\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
